Distributionally Robust Bayesian Quadrature Optimization

Bayesian quadrature optimization (BQO) maximizes the expectation of an expensive black-box integrand taken over a known probability distribution. In this work, we study BQO under distributional uncertainty in which the underlying probability distribution is unknown except for a limited set of its i.i.d. samples. A standard BQO approach maximizes the Monte Carlo estimate of the true expected objective given the fixed sample set. Though Monte Carlo estimate is unbiased, it has high variance given a small set of samples; thus can result in a spurious objective function. We adopt the distributionally robust optimization perspective to this problem by maximizing the expected objective under the most adversarial distribution. In particular, we propose a novel posterior sampling based algorithm, namely distributionally robust BQO (DRBQO) for this purpose. We demonstrate the empirical effectiveness of our proposed framework in synthetic and real-world problems, and characterize its theoretical convergence via Bayesian regret.

==> body/appnedixD.tex <==
\section*{Appendix D}
For the details of derivation for posterior sampling (a.k.a Thompson sampling), see Appendix A of \cite{nipsMuandetFDS12}. 

==> body/drbo.tex <==
\section{Distributionally robust Bayesian quadrature optimization}

\huong{I find it really hard to follow this section. You need to have a paragraph here to summarize the core idea of your work. Read Rule 23 in the email I just forwarded to you.}

\subsection{Distributional uncertainty set}
% In this work, we assume that $f$ is bounded, i.e., $\exists B_0, \exists B_1, f(x,w) \in [B_0, B_1], \forall x \in \mathcal{X}, w \in \Omega$. 
\begin{defn}[$\phi$-divergence]
For a convex function $\phi: \mathbb{R}_{+} \rightarrow \mathbb{R}$ with $\phi(1) = 0$, the $\phi$-divergence between two probability measures $P$ and $Q$ defined on $\mathcal{X}$ is: 
\begin{align*}
    D_{\phi}(p \| q) = \int_{\mathcal{X}} \phi \left(\frac{dp}{dq} \right)dq.
\end{align*}
\end{defn}
\huong{Citation? For each concept, definition, you need to make it clear if it's your newly-introduced concept, or if it is presented in some other works.}
\huong{Also, before presenting any new definition, theorem, etc., need to explain why those concepts are needed, and where they are in the whole picture of the paper. This helps to make the readers to be able to link everything together and be able to understand your work.}
In this paper, we focus on $\chi^2$-divergence which is a $\phi$-divergence with $\phi(t) = \frac{1}{2}(t-1)^2$ \huong{Why this specific divergence?}. We define an uncertainty distributional set centered around the empirical distribution $\hat{p}_n$ wrt $\chi^2$-divergence: 
\begin{align}
    \label{eq:uncertainty_set}
    \mathcal{P}_{n,\rho} := \left\{ p \in \mathcal{P}: D_{\phi}(p \| \hat{p}_n) \leq \rho \right\} \nonumber \\ 
    = \left\{  \sum_{i=1}^n p_i \delta(w - w_i) \bigg| p \in \Delta_n,  n \|p\|_2^2 \leq 2\rho +1 \right\}
\end{align}
\huong{Use $\&$ in the above equation to align the two '='.}
where $\Delta_n = \{u = (u_1, ..., u_n) \in \mathbb{R}_{+} | u^T \pmb{1}_n = 1 \}$ is the $n$-dimensional simplex and $\pmb{1}_n$ is the $n$-dimensional vector of ones. 
\begin{defn}[$\rho$-robust conditional quadrature weights]
The $\rho$-robust conditional quadrature weights for any function $u: \mathcal{X} \times \mathcal{W} \rightarrow \mathbb{R}$ is defined as $p_{u,\rho}(. |x) := \argmin_{p \in \mathcal{P}_{n, \rho}} \mathbb{E}_{p(w)}[u(x,w)], \forall x \in \mathcal{X}$. 
\end{defn}


We then define the \textit{distributional robust counterpart} of Eq. (\ref{eq:stochastic_opt}) as 
\begin{align}
    \label{eq:dr}
    g_{\rho}(x) &= \min_{p\in \mathcal{P}_{n, \rho}} \mathbb{E}_{p(w)}[f(x,w)] = \mathbb{E}_{p^{f, \rho}_x}(w) [f(x,w)]
\end{align}

% Note that if $f$ is a stochastic process, $p^*_x$ are also stochastic. However, since $f$ is a unknown and deterministic function, we bui


% Note that given a fixed (but unknown) objective $f$, the optimal distributions $P^*_x, \forall x \in \mathcal{X}$ are also fixed and unknown. If $f$ is a stochastic process, the optimal distribution $P^*_x, \forall x \in \mathcal{X}$ are also stochastic processes. In Bayesian optimization, $f$ is a fixed (but unknown) function. Thus, we still keep fixed the unknown optimal distributions $P^*_x$ even we assume a probabilistic model over $f$ to model its uncertainty during information gathering. In this sense, $G_{\rho}(x)$ is a linear transformation of $f$ with deterministic weights $P^*_x, \forall x \in \mathcal{X}$; thus it follows a GP if $f \sim GP$. 

The distributional robust counterpart is equivalent to the variance-regularized objective $g_{bv}(x)$ when the sample variance is high, as guaranteed by the following theorem: 
\begin{thm}[\cite{nipsNamkoongD17}]
Let $Z \in [B_0, B_1]$ be a random variable (e.g., $Z = f(x,w)$ for a fixed $x$), a fixed $\rho \geq 0$, $B = B_1 - B_0$, and $s_n^2 = Var_{\hat{p}_n}[Z]$, we have: 
\begin{align*}
    &\max \left\{ \sqrt{2\rho s^2_n} - 2B\rho, 0 \right\}
    \leq \\
    &\mathbb{E}_{\hat{p}_n}[Z] - \inf_{p} \left\{  \mathbb{E}_{p}[Z]:  p \in  \mathcal{P}_{n,\rho} \right\}
    \leq \sqrt{2\rho s^2_n}.
\end{align*}
\end{thm}

In addition, the distributional robust counterpart also covers the Monte Carlo estimate or the worst-case estimate for special values of the uncertainty radius $\rho$ as stated in the following proposition:
\begin{prop} Given $g_{\rho}$, $g_{mc}$, and $g_{wc}$ are defined in Eq. (\ref{eq:dr}), (\ref{eq:mc}), and (\ref{eq:wc}), respectively, we have:
\begin{align}
g_{\rho}(x) = 
    \begin{cases}
        g_{mc}(x) \text{ if } \rho = 0, \\
        \min_{w \in S_n} f(x,w) \text{ if } \rho \geq \frac{n-1}{2}.
    \end{cases} \nonumber
\end{align}
\end{prop}



% Therefore, instead of directly optimizing (\ref{eq:variance_reg}), we propose the $\rho$-robust optimization problem as maximization of the distributionally robust counterpart: 
% \begin{align}
%     \label{eq:dr_minmax}
%     \max_{x \in \mathcal{X}} g_{\rho}(x) &= \max_{x \in \mathcal{X}} \min_{\hat{p} \in \mathcal{P}_{n, \rho}} \mathbb{E}_{\hat{p}(w)}[f(x,w)] = \max_{x \in \mathcal{X}} \mathbb{E}_{p^{*}_{x}(w)}[f(x,w)] 
% \end{align}

\subsection{Gaussian Process on distributionally robust quadrature}
We build a GP over $f$. To eliminate confusion, we denote the deterministic $f$ by $f_0$, and the Gaussian stochastic process over $f_0$ by $f$. Note that since $f$ is a stochastic process, $g_{\rho}$ is not a GP anymore because $p^{f,\rho}_x$ depends on $f$. Instead, we consider:
\begin{align}
    g_{\rho,f_0}(x) &:= \mathbb{E}_{p^{f_0, \rho}_x} [f(x,w)]. \nonumber
\end{align}
then $g_{\rho,f_0}(x)$ is a GP. The main challenge is however the $\rho$-quadrature weights $p^{f_0, \rho}_x$ associated with $f_0$ are unknown. 

% However, since originally $f_0$ is deterministic (but unknown), we assume that $p^{f,\rho}_x$ is computed on the deterministic $f_0$, not the $f$ from GP; thus denote it by $p^{f_0,\rho}_x$. In this sense, $g_{\rho}$ is a GP with unknown quadrature weights $p^{f_0,\rho}_x$. Thus, the main challenge is to infer such unknown quadrature weights at every iterations when we query a new observation of $f$. 

To overcome this challenge, we propose to use the $\rho$-quadrature weights of a posterior function sample of $f$ as a surrogate $\rho$-quadrature weights of $f_0$. The surrogate $\rho$-quadrature weights are then used to select new samples using a quadrature acquisition. The rationale for this approach is that as the iteration approaches infinity, the posterior function sample approaches the true function $f$, thus the estimated quadrature weights approaches the true quadrature weights. 


% The main challenge is to solve the minmax problem (\ref{eq:dr_minmax}) efficiently under a limited budget of function evaluations. To solve the minmax black-box optimization, we introduce \textit{distributionally robust knowledge gradient} (DRKG) policy. This is a variant of KG that computes distributional robust weights. 

% \subsubsection{Knowledge Gradient}

% \begin{equation}
%     \texttt{quadKG}(x_{n+1}, w_{n+1}) = \mathbb{E}_n \left[\max_{x \in \mathcal{X}} \mathbb{E}_{\hat{p}(w)} \left[ a_{n+1}(x, w; x_{n+1}, w_{n+1}) \right] \right] - \max_{x \in \mathcal{X}} \mathbb{E}_{\hat{p}(w)} \left[ a_n(x, w) \right] 
% \end{equation}
% where 
% \begin{align*}
%     a_{n+1}(x, w; x_{n+1}, w_{n+1}) = a_n(x, w) + Z b_n(x,w;  x_{n+1}, w_{n+1}) \\
%     a_n(x, w) = 
%      \begin{bmatrix}
%      \Sigma_0(x,w;x_1, w_1) & \hdots & \Sigma_0(x,w;x_n, w_n) 
%      \end{bmatrix} K_n^{-1}  
%      \begin{bmatrix}
%      y_1 \\
%      \vdots \\
%      y_n
%      \end{bmatrix}  \\
%      \gamma^T =  \begin{bmatrix}
%      \Sigma_0( x_{n+1}, w_{n+1};x_1, w_1) & \hdots & \Sigma_0( x_{n+1}, w_{n+1};x_n, w_n) 
%      \end{bmatrix}
% \end{align*}
% \begin{align*}
%     b_n(x,w;  x_{n+1}, w_{n+1}) = \frac{
%      \Sigma_0(x,w ;x_{n+1}, w_{n+1}) - 
%      \begin{bmatrix}
%      \Sigma_0(x,w;x_1, w_1) & \hdots & \Sigma_0(x,w;x_n, w_n) 
%      \end{bmatrix} K_n^{-1} \gamma 
%      }{
%      \sqrt{
%      \Sigma_0(x_{n+1}, w_{n+1}; x_{n+1}, w_{n+1}) - \gamma^T K_n^{-1} \gamma + \lambda(x_{n+1}, w_{n+1})
%      }
%      }
% \end{align*}
% if $\lambda(x_{n+1}, w_{n+1}) >0$  or  
% $(x_{n+1}, w_{n+1}) \notin \{(x_i, w_i): 1 \leq i \leq n\}$; and $ b_n(x,w;  x_{n+1}, w_{n+1}) =0$ otherwise.  

% \subsubsection{Distributional Robust Knowledge Gradient}

% \begin{equation}
%     \texttt{DRKG}(x_{n+1}, w_{n+1}) = \mathbb{E}_n \left[\max_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{n, \rho}}\mathbb{E}_{\hat{P}} \left[ a_{n+1}(x, w; x_{n+1}, w_{n+1}) \right] \right] - \max_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{n, \rho}}\mathbb{E}_{\hat{P}} \left[ a_n(x, w) \right]
% \end{equation}

% The distributional robust objective and its gradient can be computed analytically by solving the KKT conditions for the Lagrangian multiplier. 


\subsection{The optimal $\rho$-robust quadrature weights}
\label{subsec:robust_quad_weights}
We consider the optimal $\rho$-robust quadrature weight problem in which given $l = (l_i)_{i=1}^n$, we solve the constrained minimization problem: $\min_{p \in  \mathcal{P}_{n,\rho}} p^T l$
% \begin{align}
%     \label{eq:rho_quadrate_weights}
%     \min_{p \in  \mathcal{P}_{n,\rho}} p^T l
% \end{align}
where $\mathcal{P}_{n,\rho}$ is defined in Eq. (\ref{eq:uncertainty_set}). 
\begin{prop}
Comment: in our case, minimax is not necessarily equal to maximin but that does not affect the result in our work. \cite{NamkoongD16} applies to solve for convex $f$ but in our case we solve for any function $f$ and compute the exact inner min value and its gradients. This inner min is smooth and differentiable (?) [but even not, we still can use DIRECT?]
\begin{align*}
    \begin{cases}
    n \lambda &= \sum_{i=1}^n (-l_i - \eta)_{+} \\ 
    \eta &= \frac{-\sum_{i \in A} l_i - n \lambda}{ |A|} \\ 
    A &= \{ i: l_i + \eta \leq 0  \} \\ 
       \frac{\partial p_i}{\partial \psi}  &= \frac{-1}{n \lambda^2} (-l_i - \eta) \frac{\partial \lambda}{\partial \psi}  + \frac{1}{n \lambda}(-\frac{\partial l_i}{\partial \psi} -\frac{\partial \eta}{\partial \psi}) \\
    |A| \frac{\partial \eta}{\partial \psi} &=  -\sum_{i \in S} \frac{\partial l_i}{\partial \psi} - n \frac{\partial \lambda}{\partial \psi} \\ 
    \sum_{i \in S} p_i \frac{\partial p_i}{\partial \psi} &= 0.  
    \end{cases}
\end{align*}

%  \begin{align}
%  \begin{cases}
%     \label{eq:dr_gradient}
%     \frac{\partial p_i}{\partial \psi}  = \frac{-1}{n \lambda^2} (-l_i - \eta) \frac{\partial \lambda}{\partial \psi}  + \frac{1}{n \lambda}(-\frac{\partial l_i}{\partial \psi} -\frac{\partial \eta}{\partial \psi}) \\
%     |A| \frac{\partial \eta}{\partial \psi} =  -\sum_{i \in S} \frac{\partial l_i}{\partial \psi} - n \frac{\partial \lambda}{\partial \psi} \\ 
%     \sum_{i \in S} p_i \frac{\partial p_i}{\partial \psi} = 0.      
%  \end{cases}
%  \end{align}
\end{prop}


\subsection{Algorithmic Approach}
\begin{algorithm}
\DontPrintSemicolon
  
\KwInput{Prior \texttt{GP}($\mu_0$, $\Sigma_0$), horizon $T$, fixed sample set $S_n$, distributional confidence $\rho$.}
%   \KwInitialization{$\theta$}

    \For{$t = 1$ to $T$}    
    { 
    \tcc{posterior sampling}
    Sample $\tilde{f}_t \sim $ \texttt{GP}$\left(\mu_{t-1}, \Sigma_{t-1}\right)$. \; %\Comment{\textcolor{blue}{posterior sampling}} \; 
    
    \tcc{$\rho$-robust quadrature weights}
    Choose $\displaystyle x_t \in \argmax_{x \in \mathcal{X}} \min_{p \in \mathcal{P}_{n,\rho}}  \mathbb{E}_{p(w)} [\tilde{f}_t(x,w)]$. \; 
    
    \tcc{highest posterior variance}
    Choose $ \displaystyle w_t = \argmax_{w \in S_n} \Sigma_{t-1}(x_t, w; x_t, w)$. \; %\Comment{\textcolor{blue}{highest posterior variance}} \;
    
    Observe reward $\hat{y}_t \leftarrow f(x_t, w_t) + \epsilon_t$. \;
    
    Perform update \texttt{GP} to get $\mu_{t}$ and $\Sigma_{t}$.}

\KwOutput{$\displaystyle \argmax_{ x \in \{x_1, ..., x_T\}} \min_{p \in \mathcal{P}_{n,\rho}}  \mathbb{E}_{p(w)} [\mu_T(x,w)]$.}
\caption{\texttt{DRBQO}: Two-player Bayesian quadrature optimization}
% \label{alg:drbopt}
\label{pseudo_code:acq}
\end{algorithm}


Note that for any function $\tilde{f}_t(x,w)$, we can compute the exact value and gradient wrt $x$ of $\min_{p \in \mathcal{P}_{n,\rho}}  \mathbb{E}_{p(w)} [\tilde{f}_t(x,w)]$ using the optimal $\rho$-robust quadrature weights in the previous subsection. The intuition behind the optimal $\rho$-robust quadrature weights is to seek for a robust solution that accounts for the most adversarial distribution of the quadrature. The parameter $\rho \geq 0$ controls the degree of conservative for the robust solution. For one extreme case where $\rho=0$, the $\rho$-robust quadrature weights reduce to the empirical ones $p_i = 1/n, \forall 1 \leq i \leq n$. For the other extreme case where $\rho \geq \frac{n-1}{2}$, the optimal quadrature weights has only one non-zero component. 


% \begin{align}
%     \label{eq:eta_to_lam}
    
% \end{align}

% From Eq. (\ref{eq:eta_to_lam}), we have:
% \begin{align}
%     \label{eq:lam_to_eta}
    
% \end{align}

% from subsection \ref{subsec:robust_quad_weights}. 

% \begin{algorithm}
% \caption{Two-player distributional robust \texttt{BQO}}\label{alg:drbopt}
% \begin{algorithmic}[1]
% \Procedure{\texttt{DRBQO}}{$\Sigma_0$, $\mu_0$, $D_0$, $T$, $S_n$, $\rho$}
% \For{$t=1,2,..., T$}
% \State $\tilde{f}_t \sim $ GP posterior of $f$. \Comment{Posterior sampling.}
% \State $x_t \in \argmax_{x \in \mathcal{X}} \min_{p \in \mathcal{P}_{n,\rho}}  \mathbb{E}_{p(w)} [\tilde{f}_t(x,w)]$. \Comment{ The inner minimization has a closed form and exact gradient from Subsection \ref{subsec:robust_quad_weights}}
% \label{pseudo_code:acq}
% % EXTENSION: know p but would like to perform maximin here.  Instead of sample p, because the number of samples is large, we need to do some thing more clever, e.g., Statement: given max_{x} min_{p} E_{p(w)}[f(x,w)] and that you can sample p. What is the best way to reduce variance? Can we still do maximin around w_i we sample? That's what I am experimenting with. 
% \State $\displaystyle w_t = \argmax_{w \in S_n} \sigma_n(x_t, w)$. \Comment{Choose $w_t$ at the highest posterior variance}
% \State $\hat{y}_t \leftarrow f(x_t, w_t) + \epsilon_t$.
% \State $D_t = D_{t-1} \cup \{x_t, w_t, \hat{y}_t\}$.
% \State Update GP using $D_t$.
% \EndFor
% \Return $\displaystyle x_{\tau}$ where $\tau := \argmax_{ 1 \leq t \leq T} \min_{p \in \mathcal{P}_{n,\rho}}  \mathbb{E}_{p(w)} [\tilde{f}_T(x_t,w)]$.
% \EndProcedure
% \label{alg:dropt}
% \end{algorithmic}
% \end{algorithm} 
 

% \ref{pseudo_code:acq}
 
% Assume $f$ follows a Gaussian process with a Gaussian prior: 
% \begin{align*}
%     f | \mathcal{F}_n \sim \texttt{GP}(\mu_n, \Sigma_n), \forall n \geq 0,
% \end{align*}
% where $\mathcal{F}_n = \{ x_0, w_0, \hat{y}_1, ..., x_{n-1}, w_{n-1}, \hat{y}_n  \}$ is the acquired observations at time $n$. Since $\hat{g}_{DR}$ is a linear function of $f$, $G_{\rho}$ is also a Gaussian process with:
% \begin{align*}
%     \mu_{n, \rho}(x) &:= \mathbb{E}\left[G_{\rho}(x) | \mathcal{F}_n \right] = \int \mu_n(x, w) dP^*_x(w)\\
%     \Sigma_{n, \rho}(x,x') &:= \texttt{Cov} \left[G_{DR}(x), G_{DR}(x') | \mathcal{F}_n \right]  = \int \int \Sigma_n(x,w, x', w') dP^*_x(w) dP^*_x(w')
% \end{align*}
% We then define Distributionally Robust Bound (DRB) for $G$

% \begin{equation}
%     \texttt{DRB}_t(x) = \inf_{\hat{P} \in \mathcal{P}_{m, \rho}} \left( \int \mu_t(x,w)d\hat{P}(w) + \beta_{t+1}^{1/2} \int \sigma_t(x, w) d\hat{P}(w) \right)
%     % \texttt{drb}_t(x) = \inf_{\hat{P} \in \mathcal{P}_{m, \rho}} \left( \int \mu_t(x,w)d\hat{P}(w) + \beta_{t+1}^{1/2} \int \int \Sigma_t(x, w, x, w') d\hat{P}(w) d\hat{P}(w') \right)
%     \label{eq:drb}
% \end{equation}
% \thanh{Eq. \ref{eq:drb} does not consider correlation between $w_i$. For an application to cross-validation, it might be beneficial to consider such correlation. }
% \begin{algorithm}
% \caption{The \texttt{DROpt} algorithm.}\label{alg:dropt}
% \begin{algorithmic}[1]
% \Procedure{\texttt{DROpt}}{$\Sigma_0$, $\mu_0$, $T$, $\{\beta_t\}_{t=1}^T$}
% \For{$t=1,2,..., T$}
% \State $\displaystyle x_t \in \argmax_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{m, \rho}} \mathbb{E}_{\hat{P}} [\texttt{ucb}_{t-1}(x,w)]$ \Comment{$\texttt{drb}_{t-1}$ computes Eq.~\ref{eq:drb}}
% \State $\displaystyle w_t = \argmax_{w \in W} \sigma_n(x_t, w)$ 
% \State $\displaystyle \hat{y}_t \leftarrow \text{Query } f \text{ at } (x_t, w_t)$
% \State Update $\mu_t$, $\Sigma_t$, and $\texttt{drb}_t$ by including $\{(x_t, w_t, \hat{y}_t)\}$
% \EndFor
% \Return $\displaystyle x^*_{T} := \argmax_{x_t, 1 \leq t \leq T}  \texttt{drb}_{t-1}(x_t)$
% \EndProcedure
% \label{alg:dropt}
% \end{algorithmic}
% \end{algorithm}

% It remains to solve the minimax optimization of the DRB acquisition function (line 3 at Algorithm \ref{alg:dropt}). We try with the two-player bandit mirror which alternates between gradient descent steps on $p$ and sub-gradient ascent on $l$: 
% \begin{algorithm}
% \caption{The two-player bandit mirror descent algorithm.}\label{alg:mirror_descent}
% \begin{algorithmic}[1]
% \Procedure{\texttt{MirrorDescent}}{$T$, $\alpha_x$, $\alpha_p$, $x_1$, $p_1 = \mathbf{1}/m$}
% \For{$t=1,2,...,T$}
% \State $I_t \sim p_t$
% \State $\hat{l}_{t,i}(x) = \frac{l_i(x)}{p_{t,i}}\mathbf{1}\{I_t=i\}$
% \State $$
% \EndFor
% \Return $\displaystyle x^*_{T} := \argmax_{x_t, 1 \leq t \leq T}  \texttt{drb}_{t-1}(x_t)$
% \EndProcedure
% \label{alg:dropt}
% \end{algorithmic}
% \end{algorithm}


% \subsection{Analysis}
% We define $\rho$-regret: 
% \begin{equation}
%     r_{\rho}(x_t) := \max_{x \in \mathcal{X}} \mathbb{E}_{P}[f(x, w)] - \min_{\hat{P} \in \mathcal{P}_{m, \rho}} \mathbb{E}_{\hat{P}}[f(x_t, w)] = d_{\rho} + \hat{r}_{\rho}(x_t)
% \end{equation}
% where 
% \begin{equation}
%     d_{\rho} := \max_{x \in \mathcal{X}} \mathbb{E}_{P}[f(x, w)] - \max_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{m, \rho}} \mathbb{E}_{\hat{P}}[f(x, w)]
% \end{equation}
% \begin{equation}
%     \hat{r}_{\rho}(x_t) := \max_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{m, \rho}} \mathbb{E}_{\hat{P}}[f(x, w)] - \min_{\hat{P} \in \mathcal{P}_{m, \rho}} \mathbb{E}_{\hat{P}}[f(x_t, w)]
% \end{equation}

% \begin{thm} (Upper bound)
% Fix $\rho > 0$, $\epsilon > 0$, $\delta \in (0,1)$, $T \in \mathbb{N}$, $C_1 = 8 / \log(1 + \sigma_g^{-2})$, $\gamma_t$ is the maximum information gain of $\hat{g}_{DR}$ up to time $t$, and $\beta_t = (B + \sigma_g \sqrt{2(\gamma_{t-1} + \log \frac{e}{\delta})})^2$ then we have, with probability at least $1-\delta$
% \begin{equation}
%     \hat{r}_{\rho}(x^*_T) \leq \sqrt{ \frac{C_1 \beta_T \gamma_T}{T} }
% \end{equation}
% \end{thm}
% \thanh{With the assumption that $f$ is i.i.d. corrupted by a Gaussian noise $\sigma_f$, how can we derive an equivalent $\sigma_g$ for $g$?}

% \thanh{Can we prove, or at least argue, that the minimax problem in line 4 exists solution, at least for a bounded domain?}

% \begin{proof}[\textbf{Proof}]

% \begin{align*}
%     \hat{r}_{\rho}(x_t) 
%     &= \max_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{n, \rho}} \mathbb{E}_{\hat{P}}[f(x, w)] - \min_{\hat{P} \in \mathcal{P}_{n, \rho}} \mathbb{E}_{\hat{P}}[f(x_t, n)] \\ 
%     &\leq \max_{x \in \mathcal{X}} \min_{\hat{P} \in \mathcal{P}_{n, \rho}} \mathbb{E}_{\hat{P}}[\texttt{UCB}_{t-1}(x, w)] - \texttt{LCB}^G_{t-1}(x_t) \\ 
%     % &\leq  \max_{x \in \mathcal{X}} \texttt{drb}_{t-1}(x) - \texttt{lcb}^g_{t-1}(x_t) \\ 
%     &= \texttt{DRB}_{t-1}(x_t) - \texttt{LCB}^g_{t-1}(x_t) \\ 
%     &\leq \mathbb{E}_{P^*_{x_t}}[\mu_{t-1}(x_t, w)] + \beta_t \mathbb{E}_{P^*_{x_t}}\mathbb{E}_{P^*_{x_t}}[ \Sigma_{t-1}(x_t, w, x_t, w')] - \texttt{LCB}^G_{t-1}(x_t) \\ 
%     &= \mu_{t-1}^G(x_t) + \beta_t^{1/2} \sigma_{t-1}^G(x_t) - (\mu_{t-1}^G(x_t) + \beta_t^{1/2} \sigma_{t-1}^G(x_t)) \\ 
%     &= 2 \beta_t^{1/2} \sigma_{t-1}^G(x_t).
% \end{align*}
% \end{proof}

